BEVFusion4D: Learning LiDAR-Camera Fusion Under Bird's-Eye-View via Cross-Modality Guidance and Temporal Aggregation

Integrating LiDAR and Camera information into Bird's-Eye-View (BEV) has become an essential topic for 3D object detection in autonomous driving. Existing methods mostly adopt an independent dual-branch framework to generate LiDAR and camera BEV, then perform an adaptive modality fusion. Since point clouds provide more accurate localization and geometry information, they could serve as a reliable spatial prior to acquiring relevant semantic information from the images. Therefore, we design a LiDAR-Guided View Transformer (LGVT) to effectively obtain the camera representation in BEV space and thus benefit the whole dual-branch fusion system. LGVT takes camera BEV as the primitive semantic query, repeatedly leveraging the spatial cue of LiDAR BEV for extracting image features across multiple camera views. Moreover, we extend our framework into the temporal domain with our proposed Temporal Deformable Alignment (TDA) module, which aims to aggregate BEV features from multiple historical frames. Including these two modules, our framework dubbed BEVFusion4D achieves state-of-the-art results in 3D object detection, with 72.0% mAP and 73.5% NDS on the nuScenes validation set, and 73.3% mAP and 74.7% NDS on nuScenes test set, respectively.

==> latex/Sections/Method_update.tex <==
\graphicspath{{\subfix{../Images/}}}
\section{Methods}


In this section, we present an overview of our proposed \name{} shown in Fig.~\ref{Fig.main}. The overall pipeline includes three stages named feature extraction, spatial fusion, and temporal fusion, respectively. We first present the feature extraction stage (Section 3.1). Then spatial fusion is presented with a detailed discussion of our LGVT module (Section 3.2). Furthermore, we describe our temporal fusion method based on the proposed TDA module (Section 3.3). In Sections 3.1 and 3.2, we refer to the process of feature extraction and spatial fusion at the current frame $T$ for simplicity. The exploration of temporal information is explained in Section 3.3.

\subsection{LiDAR and Camera Feature Extraction}
In the feature extraction stage, we adopt a dual-branch paradigm of previous works~\cite{liangbevfusion, liu2022bevfusion} to process cross-modality data. Specifically, the LiDAR point cloud and multi-view images at the current frame $T$ are fed into two independent backbones to form high-level feature representations. For the LiDAR stream, the input point clouds $P \in \mathbb{R}^{N \times D}$ is converted into a unified grid through voxelization~\cite{zhou2018voxelnet} and further processed by the 3D sparse convolution~\cite{yan2018second} to form the feature representation in the BEV space $B_{LiDAR} \in \mathbb{R}^{X \times Y \times C}$, where $X$, $Y$, $C$ represent the size of the BEV grid and feature dimensions. The image backbone takes multi-view image data to yield semantic feature representations in 2D $I \in \mathbb{R}^{N_{c} \times C\times H\times W}$, where $N_{c}$, $C$, $H$, $W$ denote the number of cameras, feature dimensions and size, respectively. Then the fusion of extracted LiDAR and image features will be carried out in the following spatial fusion stage.

\subsection{Spatial Fusion}
The extracted features of LiDAR and images deliver the essential information of geometry and semantics, respectively. To further incorporate these features into a unified BEV space, a view transformation is required to project the multiple 2D image features into Camera BEV space. Previous methods~\cite{liangbevfusion, liu2022bevfusion} choose LSS~\cite{philion2020lift} to achieve this task by lifting 2D features into 3D space with various depth probabilities. However, the absence of reliable depth supervision for this module usually results in an inferior performance. In contrast, we rely on the relatively accurate spatial information from the pretrained LiDAR BEV to acquire corresponding semantic features. This enables our proposed LGVT to effectively project the 2D image features into BEV space.

\textbf{LiDAR-Guided View Transformer Module (LGVT).} Fig.~\ref{Fig.img_BEV} shows the detail of our LGVT module, where the Camera BEV $B_{Camera}$ is recurrently updated with the guidance of LiDAR $B_{LiDAR}$. Specifically, 
Camera BEV of the previous layer $B_{Camera}^{i-1}$ is first integrated with LiDAR BEV features $B_{LiDAR}$ to achieve cross-modality query interactions and produce LiDAR-guided image query $Q_{guided}^i$.  the above process could be formulated in Eq.~\ref{eq.query concat}: 

\begin{equation}
\label{eq: query concat}
\begin{split}
    Q_{guided}^i = f(B_{LiDAR}, B_{Camera}^{i-1}), \\
    \text{where}~B_{Camera}^{i-1} = 
    \left\{\begin{matrix}
    B_{Camera}^{init},&i=1,\\
    B_{Camera}^{i-1} ,&i>1.
    \end{matrix}\right. \\
\end{split}
\end{equation}
Then a deformable cross-attention module~\cite{zhu2020deformable} takes the guided query $Q_{guided}^i$ and image features to generate updated Camera BEV in the current layer $B_{Camera}^{i}$ as shown in Eq.~\ref{eq: deform attention}.
\begin{equation}
\label{eq: deform attention}
    B_{Camera}^i = MSDeformCrossAttn(Q_{guided}^i, I),
\end{equation}
where i is the index of layers, and $MSDeformCrossAttn$ denotes multi-scale deformable attention~\cite{zhu2020deformable}. 


To facilitate the recurrent process in our LGVT module, a corresponding initialization strategy is proposed to generate Camera BEV features in the first layer. Following previous work~\cite{li2022bevformer}, we pre-define an empty BEV feature grid with a fixed height of $N_{h}$ and assign each query $(i, j)$ of the BEV plane its relevant reference points $(i, j, h_n)$ in the 3D pillar. Then these points are mapped into the 2D image features through the camera view projection as Equation~\ref{eq: project}:

\begin{equation}
    ((x_n^{1}, y_n^{1}),...,(x_n^{N_{c}}, y_n^{N_{c}})) = Project(i, j, h_n), \\
    I_{(x_n^m, y_n^m)} = Sample((x_n^m, y_n^m), I)),\\    
    \label{eq: project}
\end{equation}
where $M$ is the number of cameras, $M_{hit}$ denotes the number of valid sampling locations, $n=1,...,N, m=1,...,M$, $(x_n^m, y_n^m)$ are the coordinates in 2D image features corresponding to the at $m_{th}$ view, $Project$ and $Sample$ represents the camera projection matrix and the bilinear interpolation, respectively.

Then the image features of max response 




Specifically, for a camera BEV feature grid with coordinate $(i, j)$, we pre-defines $N$ heights $\{h_1, h_2,...,h_N\}$ for this grid and project $\{(i, j, h_1),...(i, j, h_N)\}$ to 2D multi-view image features using camera matrix. 


and sample the maximum image feature, then we concatenate the image feature with the corresponding LiDAR BEV feature grid. The process can be formulated as follows:






and fill it with the corresponding 2D image features, then concatenate it with the corresponding LiDAR BEV features. Specifically, for a camera BEV feature grid with coordinate $(i, j)$, we pre-defines $N$ heights $\{h_1, h_2,...,h_N\}$ for this grid and project $\{(i, j, h_1),...(i, j, h_N)\}$ to 2D multi-view image features using intrinsics and extrinsics, and sample the maximum image feature, then we concatenate the image feature with the corresponding LiDAR BEV feature grid. The process can be formulated as follows: 
\begin{gather}
    ((x_n^{1}, y_n^{1}),...,(x_n^{M}, y_n^{M})) = Project(i, j, h_n), \label{eq.project}\\
    I_{(x_n^m, y_n^m)} = Sample((x_n^m, y_n^m), I)),\\
    I_{(i, j)} = \frac{1}{M_{hit}}\sum_{m=1}^{M_{hit}}{\max_{n=1,...,N}(I_{(x_n^m, y_n^m)})}, \\
    B_{Camera}^{init}(i, j) = Concat(B_{LiDAR}(i, j), I_{(i, j)})
\end{gather}






\subsection{Temporal Fusion}


  







BEVFusion4D first takes 2D image features and LiDAR point clouds to generate camera BEV features and LiDAR BEV features in corresponding branches. Then BEVFusion4D fuses them into a unified BEV space representation at current time T. Finally, the present fused BEV features will be fused with aligned historical fused BEV features and turn to final temporal fused BEV feature. The final temporal-spatial fused BEV feature will be sent to the decoder to get the detection result.

Fig.~\ref{Fig.main} shows the architecture of BEVFusion4D. BEVFusion4D generates camera BEV features and LiDAR BEV features in corresponding branches. In the image branch, LiDAR BEV features are used as spatial prior to 

BEVFusion4D first takes 2D image feature $I \in \mathbb{R}^{N_{camera} \times C\times H\times W}$ and LiDAR point clouds $P \in \mathbb{R}^{N \times D}$ to generate camera BEV features $B_{camera} \in \mathbb{R}^{X \times Y \times C} $ and LiDAR BEV features $B_{LiDAR} \in \mathbb{R}^{X \times Y \times C}$ in corresponding branches. Then BEVFusion4D fuses them into a unified BEV space representation $F^T \in \mathbb{R}^{X \times Y \times C}$ at current time T. Finally, the present fused BEV features $F^T$ will be fused with aligned $n$ historical fused BEV features $\{F^{T-1},..., F^{T-n}\}$ and turn to final temporal fused BEV feature $F^{T}_{temporal}$. The final temporal-spatial fused BEV feature $F^{T}_{temporal}$ will be sent to the decoder to get the detection result.
\begin{figure}[htb]
\centering
\includegraphics[scale=0.35]{latex/Images/bev_compare.pdf}
% \includegraphics[width=1\textwidth,height=0.4\textwidth]{latex/Images/temporal_BEV.pdf}
\caption{We visualize Camera and LiDAR BEV features generated by BEVFusion\cite{liangbevfusion} and our framework. It is obvious that our image BEV feature is similar to the LiDAR BEV feature, which means LiDAR spatial prior plays a vital role to guide camera BEV features to generate.}
\label{Fig.bev_compare} 
\end{figure}
\begin{figure*}[htb]
\centering
% \includegraphics[scale=0.4]
\includegraphics[width=1\textwidth,height=0.4\textwidth]{latex/Images/img_BEV_branch.pdf}
\caption{(a) is the architecture of LGVT. (b) is the process of camera BEV features initialization, different colors on $B^{init}_{Camera}$ represents pre-defined heights and circles on multi-view features are the sampling location computed by Eq.~\ref{eq.project}}
\label{Fig.img_BEV} 
\end{figure*}
\subsection{LiDAR to BEV}
The LiDAR branch is responsible for converting point clouds into LiDAR BEV features. Therefore any LiDAR backbone, such as VoxelNet, CenterPoint, and PointPillar, that can generate LiDAR voxels or BEV features is compatible with our framework. As standard practice in \cite{liangbevfusion,liu2022bevfusion,bai2022transfusion,yang2022deepinteraction}, we choose VoxelNet as our LiDAR backbone to generate LiDAR BEV features.

\subsection{Camera to BEV}
The image branch is responsible for converting 2D image features into camera BEV features. BEVFusion uses LSS~\cite{philion2020lift} to generate camera BEV features, which relies on depth estimation. Fig.~\ref{Fig.bev_compare} shows the camera BEV features generated by BEVFusion\cite{liangbevfusion}, which is hard to figure out the target's location. As we import LiDAR BEV features as spatial prior to generating camera BEV features, the scene outline and targets' location can be easily distinguished as shown in our camera BEV feature.





\subsection{LiDAR-Camera BEV Features Fusion}
There are several basic ways to conduct BEV features fusion, such as concatenating, adding, and multiplying. Due to our camera BEV features inheriting spatial location information of LiDAR BEV features, camera BEV features are closer to LiDAR BEV features in space. Thus we concatenate the LiDAR and camera BEV features and send the result to convolution layers. The fusion process can be formulated as follows:
\begin{equation} \label{eq:spatialFusion}
    F = Conv(Concat(B_{LiDAR},B_{Camera})).
\end{equation}

\subsection{Temporal BEV Features Fusion}
\begin{figure}[htbp]
\centering
\includegraphics[scale=0.35]{latex/Images/temporal_BEV.pdf}
% \includegraphics[width=1\textwidth,height=0.4\textwidth]{latex/Images/temporal_BEV.pdf}
\caption{Temporal BEV features fusion module. The red and orange squares represent moving and stationary objects, respectively, while the arrows indicate the direction of the object's movement. The static align module is the alignment process formulated by Eq.~\ref{eq.alignment}.}
\label{Fig.motion_smear} 
\end{figure}

The target's historical location and orientation information is beneficial for its current motion estimation. Besides, although the BEV feature can better detect vehicles with cross-traffic, remote or near targets will still be partially out of the sensors' view, temporal information can also make up for the loss of target view loss. BEVFusion4D leads a temporal fusion on the historical fused BEV features.

Fig.~\ref{Fig.temporal_bev} shows the architecture of our temporal BEV features fusion module. Fused BEV features stored in chronological order are denoted as $\{F^{T-n},..., F^{T}\}$.  Due to each historical fused BEV feature being augmented independently, BEVFusion4D first recurrently aligns all augmented historical fused BEV features $\{F^{T-n},..., F^{T-1}\}$ in spatial and then aligns each BEV feature $F^{t}$ with the next BEV features $F^{t+1}$ based on the motion information of the ego vehicle in temporal. This alignment process can be described by the following formula:
\begin{equation} \label{eq.alignment}
    \Tilde{F}^t = K_{motion}^{t}~K_{aug}^{t}~F^t, t={T-n},...,{T-1}.
\end{equation}

The matrix $K_{motion}^{t}$ and $K_{aug}^{t}$ are termed as ego-motion transformation matrix and augment transformation matrix aligned with $F^{t+1}$ at time $t$ respectively.

As shown in Fig.~\ref{Fig.motion_smear}, the alignment process described by Eq.~\ref{eq.alignment} is limited to aligning stationary objects due to the lack of motion information. Consequently, moving objects may exhibit motion smear without any calibration, and as historical BEV features increase, the motion smear effect can become more pronounced. 

\textbf{Temporal Deformable Alignment}. To alleviate this challenge, we recurrently adopt the deformable attention mechanism to establish the correspondence between consecutive frames. The deformable attention mechanism is designed to adaptively learn the receptive field, thus enabling it to effectively capture the salient features of moving objects in the aligned BEV features. By exploiting the deformable attention mechanism, we can significantly reduce the motion smear and enhance the accuracy of the alignment process. We propose the Temporal Deformable Alignment(TDA) to conduct temporal fusion specific to moving objects.

We denote $\Tilde{F}, \hat{F}$ as BEV features static aligned by Eq.~\ref{eq.alignment} and temporal fused by TDA, respectively. Firstly, TDA concatenate two consecutive static aligned frames $\Tilde{F}^{t-1}$ and $\Tilde{F}^{t}$ as $\Tilde{F}^{t-1,t}$. We then apply the deformable attention mechanism to obtain $\hat{F}^{t-1}$ and $\hat{F}^{t}$ by using $\Tilde{F}^{t-1,t}$ as the query and $\Tilde{F}^{t-1}$, $\Tilde{F}^{t}$ as values. Next, TDA compute the average of $\hat{F}^{t-1}$ and $\hat{F}^{t}$ element-wise to update frame $\Tilde{F}^t$ by adding it to frame $\Tilde{F}^t$. The updated frame $\Tilde{F}^t_{temporal}$ can then be used for the fusion of the subsequent BEV feature. The process can be formulated as follows:
\begin{gather}
    \Tilde{F}^{t-1,t} = Concat(\Tilde{F}^{t-1}, \Tilde{F}^{t}), \\
    \hat{F}^{t-1} = DeformAttn(\Tilde{F}^{t-1,t},\Tilde{F}^{t-1}), \\
    \hat{F}^{t} = DeformAttn(\Tilde{F}^{t-1,t},\Tilde{F}^{t}), \\
    \Tilde{F^t}_{temporal} = \Tilde{F^t} + Average(\hat{F}^{t-1}, \hat{F}^{t}).
\end{gather}
where $t=2,...,T$.

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.5]{latex/Images/motion_smear.pdf}
% \includegraphics[width=1\textwidth,height=0.4\textwidth]{latex/Images/temporal_BEV.pdf}
\caption{(a) shows aligned fused BEV features $\Tilde{F}^{T-4}$ and $\Tilde{F}^T$. The red and yellow squares represent two moving objects, respectively. The arrow indicates the direction of the object's movement. (b) shows the result of different ways of temporal fusion, simply concatenating {$\Tilde{F}^{T-4},...,\Tilde{F}^T$} will cause motion smear, while our method can alleviate this effect.}
\label{Fig.motion_smear} 
\end{figure}

==> latex/Tables/FOV_module.tex <==
\begin{table}[!tb]	
\centering
\caption{Comparisons on the  }
\vspace{0.2cm}
\label{table:abl_fov}
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{l|cl|cl}
\hline
& \multicolumn{2}{c}{BEVFusion\cite{liangbevfusion}} & \multicolumn{2}{c}{Ours}\\
\hline
FOV & mAP & NDS  & mAP  & NDS \\  
 \hline
 $(-\pi/3. \pi/3)$ &  &    &      &   \\  
 \hline
 $(-\pi/2. \pi/2)$ &  &    &      &   \\  
 \hline
\end{tabular}
\end{table}



